Sum of Squares Lower Bounds from Pairwise Independence

We prove that for every $\epsilon>0$ and predicate $P:\{0,1\}^k\rightarrow \{0,1\}$ that supports a pairwise independent distribution, there exists an instance $\mathcal{I}$ of the $\mathsf{Max}P$ constraint satisfaction problem on $n$ variables such that no assignment can satisfy more than a $\tfrac{|P^{-1}(1)|}{2^k}+\epsilon$ fraction of $\mathcal{I}$'s constraints but the degree $\Omega(n)$ Sum of Squares semidefinite programming hierarchy cannot certify that $\mathcal{I}$ is unsatisfiable. Similar results were previously only known for weaker hierarchies.

==> closure-stoc.tex <==
\section{Closed sets, and the definition of the pseudo-expectation} \label{sec:closure-stoc}


%%
%Let $\I$ be a collection of \bnote{as mentioned, I think no need to talk about $P$ at all - simply about tuples of clauses} clauses $C_1, C_2, \ldots, C_m \subseteq [n]$ with a typical constraint hypergraph $G$.

Throughout the rest of this paper we fix  $\I = (C_1,\ldots,C_m)$ to be tuple of clauses of literals over $x_1,\ldots,x_n$ which is \emph{nice} in the sense that, treating $\I$ as a hypergraph,
it has $\Omega(\sqrt{\log n})$ girth. See Appendix~\ref{sec:prelims} for a more formal definition, where we also note that there exists such an $I$ that satisfies Item~2 of Theorem~\ref{thm:main}.
Whenever we mention edges, paths, or clauses, this will always be with respect to this hypergraph $\I$. In this section, we define a linear operator $\tE$ on $P_s^n$ over the linear space of multilinear polynomials on $\R^n$ of degree at most $s$ for some $s < \girth/2$. We will ensure that the $\tE$ so defined will satisfy $\tE[f(C(x))] = \E [f(\mu)]$ for every clause $C \in \I$ and function $f:\pmo^k\rightarrow\R$. In the next section, we will show that the $\tE$ we define here is in fact a pseudo-expectation operator on $P_d^n$ for  $d = \sqrt{\girth}/(100k)$ and thus obtain our main result. The $\tE$ operator we use was defined in previous works such as Benabbas et. al. \cite{BGMT12} and later also used by Tulsiani and Worah \cite{TW12} to study weaker LP/SDP hierarchies. Here, we give a construction of the same operator but use a slightly different way to obtain it that will be more suitable for our proof of the main result.

For every $S\subseteq [n]$, we define $\chi_S$ to be the function $\chi_S(x) = \prod_{i\in S}x_i$.
To define $\tE$ it is enough to define $\tE[ \chi_S]$ for every $|S| \leq s$ as one can then extend $\tE$ linearly to all of $P_s^n$. To do this, we define a probability distribution $\nu_X$ on every subset $X$ of the variables $[n]$ of size at most $s$, and then set $\tE[\chi_S]$ to be the expectation of $\chi_S$ under $\nu_S$. We make the following simple, but important definition (which is a variant of those used by prior works such as \cite{BGMT12,TW12}): (The definition and lemmas below are repeated in greater detail in Appendix~\ref{sec:closure})

\begin{definition}[Closure and closed sets] \label{def:closure:stoc} For every $R\geq 1$, a set $A\subseteq [n]$ is \emph{$R$-closed} if for every
$v,v' \in A$, if there is a path of length at most $R$ between $v$ and $v'$, then that path is contained in $A$.
We say that $A$ is \emph{closed} if it is $1$-closed.

We define the \emph{$R$-closure of $A$}, denoted by $\cl_R(A)$, to be the intersection of all sets $B$ such that $A\subseteq B$ and
$B$ is closed. The \emph{closure of $A$}, denoted by $\cl(A)$, is the $1$-closure of $A$.
\end{definition}


The following lemma (proven in the appendix) summarizes some the simple properties of the closure operation.
\begin{lemma}[Simple Properties of Closures] \label{lem:closure-props}
\begin{enumerate}
\item For every $R<\girth/2$, if $A$ and $B$ are $R$-closed and then so is $A\cap B$. Thus in particular,
$\cl_R(A)$ is an $R$-closed set for every $A$ and $R<\girth/2$.

\item For every $A$, $\cl_R(A)$ can be obtained by the following process: as long as there are $v \neq v' \in A$ of distance at most $R$ with the path between them not in $A$, add the path to $A$.
\item If $|A| < \girth/(2kR)$ then  $\cl_R(A) \leq kR|A|$.
\item If $A\subseteq B$ then $\cl_R(A)\subseteq \cl_R(B)$. %\pnote{Deleted
%something you weren't sure.  It was a leftover definition from a previous
%version.}
\item Every connected component of $\cl_R(A)$ of size $\geq 2$ intersects $A$ in at least two elements.
%\item $|\C(\cl(A))| \leq t$ and thus $|\cl(A)| \leq kt.$

\item If $A$ is closed and connected and $|A|<\girth/2$ then it is also $R$-closed for every $R < \girth/2$.
\end{enumerate}
\end{lemma}

The following lemma shows these distributions are indeed consistent:

\begin{lemma}[Consistency] \label{lem:consistent}
For every $A \subseteq B$ with $|\cl(B)| < \girth/2$, the distribution $\nu_A$
is the same as the distribution $\nu_B$ projected to $A$.
\end{lemma}

\begin{proof}[Proof sketch]
The distribution on $A$ is given as the marginal distribution of $\nu_{\cl(A)}$
on $A$, and likewise for $B$.
It suffices to check that the marginal distribution of $\nu_{\cl(B)}$ on
$\cl(A)$ equals $\nu_{\cl(A)}$.

Since $|\cl(B)|<\girth/2$, it is a forest, and $\cl(A)$ is a sub-forest of $\cl(B)$.
One can verify that it's possible to sample $\nu_{\cl(B)}$ in the following way: for
every tree $T$ in $\cl(B)$ pick an arbitrary root and set this variable to a random value in $\pmo$,
then propagate this assignment down the tree, for at each time we pick a clause $C=(v_1,\ldots,v_k)$ for which one
literal, say $v_1$, was already set to some value $a$, and sample the rest of the literals according to
the distribution $\mu|\mu_1=a$.  For every sub-tree $T'$ of $T$, the induced distribution on $T'$ is
exactly the same as the one obtained if we started from a root of $T'$, and by pairwise independence for disconnected sub-trees the distribution
is independent. Thus, the distribution on the subtrees of $\cl(B)$ corresponding to $\cl(A)$ would be
equal to $\nu_{\cl(A)}$.
\end{proof}


%\begin{corollary} \label{cor:girth-SA}
%Let $\I$ be an instance of girth $\girth$ and $\mu$ a pairwise independent
%distribution over $\{\pm 1\}^k$ such that $\girth > 4k^2$.
%Then the family of local distributions $\{\nu_X\}_{X\subseteq [n], |X| < r}$
%is an $r$-round Sherali-Adams solution for $\I$ having clause distribution
%$\mu$, where $r = \girth/(2k)-1$.
%That is,
%\begin{enumerate}
%\item Completeness: for every constraint $C$ of $\I$, $\nu_{V(C)} = \mu$
%
%\item Consistency: for every $S \subseteq T\subseteq [n]$, $|T| \leq r$, the
%marginal of $\nu_T$ on $S$ is $\nu_S$
%\end{enumerate}
%\end{corollary}
%
%\begin{proof}
%The completeness property follows from \eqref{eq:def-prob} and that $\C(V(C)) = \{C\}$.
%The consistency property follows from Lemmas~\ref{lem:closure-props} and
%\ref{lem:consistent}.
%\end{proof}
%
%\snote{Let's formally define $\pE$ here based on $\{\nu_X\}$.
%It's mentioned in the overview, but repeating the definition here won't hurt.} \pnote{Defined}

Since $\tE$ corresponds to a valid expectation locally, we obtain that $\tE$ induces a positive semidefinite (PSD) inner product on any space of functions of a small number of variables.
\begin{lemma}[Local PSDness] \label{lem:local-PSD}
Let $\tE$ be the pseudo-expectation operator for an $r$-round Sherali--Adams
solution.
Let $T$ be a subset of $[n]$ of size at most $r$.
Then for every $f\in V = \Span \{ \chi_A \mid A\subseteq T\}$, $\tE[f^2] \geq 0$.
\end{lemma}





==> prelimsBGMT.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Boaz: this file is no longer used 
%

\section{Preliminaries}

We collect some standard definitions and notation here. Let $P: \on^k \rightarrow \zo$ be any predicate of arity $k$ and let \MCSP$P$ denote $\MCSP$ CSP problem on predicate $P$. An instance $\I$ of \MCSP$P$ problem consists of $C_1, C_2, \ldots, C_m$, ordered subsets of literals on $x_1, x_2, \ldots, x_n$ of size $k$. We write $V(C_i)$ for the variables involved in the clause $C_i$. Similarly, we write $\C(V)$ for the set of all clauses $C$ such that $V(C) \subseteq V \subseteq [n]$. Constraint $C_i$ is said to be \emph{satisfied} by $x \in \on^n$ if $C_i(x) = 1$. The \emph{value} of $\I$ is the largest fraction of constraints that any assignment $x \in \on^n$ satisfies.

We will be interested in predicates that support pairwise independent distributions on their satisfying assignments:
\begin{definition}[Pairwise Independent Predicate]
A predicate $P: \on^k \rightarrow \on$ is said to be pairwise independent if there is a probability distribution $\mu$ on $P^{-1}(1) = \{ x \in \on^k \mid P(x) = 1\}$ such that $\E_{\mu}[ x_i] = 0$ and $\E_{\mu}[ x_i \cdot x_j] = 0$ for every $1 \leq i < j \leq k$.
\end{definition}

\begin{definition}[Constraint Hypergraph]
For an instance $\I$ on $n$ variables, its \emph{constraint graph} is a $k$-uniform hypergraph with the vertex set as $[n]$ and an edge for each clause containing the indices of the variables it depends on. The maximum number of edges intersecting any given edge of $G$ is said to be the \emph{degree} of $G$ and is denoted by $\Delta(G)$. The \emph{subgraph} induced by the set $A \subseteq [n]$ of vertices is defined as the hypergraph with vertex set $A$ and edges being given by the collection of all edges $e$ of $G$ such that $|e \cap A| \geq 2$. A vertex $v$ is said to be \emph{isolated} if there is no hyperedge containing it.
\end{definition}

We now define some standard ideas in the context of hypergraphs.
\begin{definition}
Let $G$ be a hypergraph. $G$ is said to be a \emph{path} if there is a sequence of hyperedges $s_1, s_2, \ldots, s_{\ell}$ such that for each $2 \leq i \leq \ell$, $s_i \cap s_{i-1} \neq \emptyset$ and $s_i \cap s_j = \emptyset$ for every $|i-j| > 1$. $G$ is said to be a \emph{cycle} if there is a path $s_1, s_2, \ldots, s_{\ell-1}$ such that there is another hyperedge $s_{\ell}$ such that $s_{\ell} \cap s_{\ell-1} \neq \emptyset$ and $s_{\ell} \cap s_1 \neq \emptyset.$ $G$ is said to be a \emph{tree} if any subset of hyperedges of $G$ do not form a cycle.
\end{definition}

\begin{definition}[Bridge Vertex in a Tree]
Let $G$ be a tree. A vertex $v$ is said to be a bridge vertex in $G$ if removing $G$ disconnects $G$ into two connected components.
\end{definition}

%For a constraint hypergraph $G$ on $n$ variables, we write $G_{\mid -S}$ to denote the graph obtained by removing $

We define the distance between two clauses in $\I$ as follows:

\begin{definition}[Distance]
The distance between two clauses $c_1$ and $c_2$ in $\I$, denoted by $\dist(c_1, c_2)$ is the minimum possible length $\ell$ of any sequence $s_1 = c_1, s_2,\ldots, s_{\ell} = c_2$ of clauses of $\I$ such that for each $2 \leq i \leq \ell$, $s_i \cap s_{i-1} \neq \emptyset$.
\end{definition}

%Next, we define a $2$-cover of a set of variables.
%\begin{definition}[$2$-Cover]
%Let $A \subseteq [n]$. Let $T_A$ be the collection of all clauses that intersect $A$ in at least $2$ elements. Let $S_A = A \setminus V(T_A)$ be the variables in $A$ not covered by the clauses in $T$. We say that $\C_A = T_A \cup S_A$ is the $2$-\emph{cover} (or simply, \emph{cover}) of $A$ in $\I$, where we view $S_A$ as a collection of singleton subsets.
%\end{definition}

Let $\I$ be an instance of \MCSP$P$ on $n$ variables and a set $\C$ of $m = \Theta(n)$ clauses. We say that $\I$ has a \emph{typical} constraint hypergraph $G$ if it satisfies:

\begin{enumerate}
\item \textbf{Low Intersection:} Any two clauses of $\I$ intersect in at most $1$ element.
\item \textbf{Acyclicity of Small Subgraphs:} For any set $A \subseteq [n]$, $|A| \leq \girth$, there is no cycle in the subgraph induced on $A$ by $G$.
%\item \textbf{Low Degree:} $\Delta(G) = O(1)$.
%\item \textbf{Small $2$-cover:} For every $A \subseteq [n]$, $|A| \leq t \leq R$, $|\C_A| \leq t+1$.
%\item \textbf{Expansion:} For every collection of at most $r$ clauses $\C$, $|\cup_{c \in \C} V(c)| \geq (k-1-\epsilon) \cdot |\C|$ for some $\epsilon < 1/3$ and $r = \Omega_{k,\epsilon}(n)$.
\end{enumerate}

\pnote{Removed expansion. We don't need it.}

It is easy to show (and well known) that the existence of an \MCSP$P$ instance with a typical constraint hypergraph. We give a proof in the Appendix \pnote{Add theorem statement here and give a proof in the appendix} for completeness.

\bnote{I believe that we just need $m=cn$ where $c$ is a large constant depending on $\e$ to ensure that for every assignment $x$ the distribution $\{ C_i(x) \}_{i \sim [m]}$ is $\e$-close to uniform}


\section{Defining $\tE$}
Let $\I$ be a collection of \bnote{as mentioned, I think no need to talk about $P$ at all - simply about tuples of clauses} clauses $C_1, C_2, \ldots, C_m \subseteq [n]$ with a typical constraint hypergraph $G$. In this section, we define a linear operator $\tE$ on $P_s^n$, \bnote{very confusing to have $N<n$: use a different letter- maybe $s$?} the linear space of multilinear polynomials on $\R^n$ of degree at most $s = \eta n$ for some constant $\eta > 0$ (depending on $k$). We will ensure that the $\tE$ so defined will satisfy $\tE[f(C_i(x))] = $ for any $f:\on^k \rightarrow \R$ and for every $1 \leq i \leq m$. In the next section, we will show that the $\tE$ we define here is in fact a pseudo-expectation operator on $P_T^n$ for $T \leq \Theta_k(\frac{\log{(n)}}{\log \log {(n)}})$ and obtain our main result. The $\tE$ operator we use was first defined by Bennabas et. al. \cite{GMT09,BGMT12} and later also used by Tulsiani and Worah \cite{TW12} to study weaker LP/SDP hierarchies. Here, we give a construction of the same operator but use a slightly different way to obtain it that will be more suitable for our proof of the main result.

To define $\tE$ it is enough to define $\tE[ \chi_S]$ for every $|S| \leq s$ as one can then extend $\tE$ linearly to all of $P_N^n$. To do this, we define a probability distribution $\nu_X$ on every subset $X$ of the variables $[n]$ of size $\eta n$ for some constant (depending on $k$) $\eta > 0$. We will then set $\tE[\chi_S]$ to be the expectation of $\chi_S$ under any $\nu_X$ such that $X \supseteq S$. The fact that $\tE[ \chi_S]$ is well-defined requires one to show that $\nu_X$ are all \emph{locally consistent}, that is, for every $X' \subseteq X_1, X_2$, the marginals of $\nu_{X_1}$ and $\nu_{X_2}$ on $X$ are equal. To define these local probability measures, we need the notion of \emph{closure} of a set of variables.




\subsection{Defining Local Probability Distributions}
We can now use the definition of closures constructed before to define local probability distributions are discussed above. \bnote{no need to talk about $P$} Let $C = (v_1, v_2, \ldots, v_k)$, where, each $v_i$ is a literal. WLOG, let $v_i \in \{x_i, -x_i\}$. We define the distribution $\mu_C$ on $V(C)$ by $\Pr_{\mu_C}[ v_1 = \eps_1, v_2 = \eps_2, \ldots, v_k = \eps_k) = \mu(x_1 = \eps_1, x_2 = \eps_2, \ldots, x_k = \eps_k)$. Then, $\mu_C$ is a pairwise independent distribution on the satisfying assignments of the clause $C$.

For every set $X \subseteq [n]$, $|X| \leq \eta n$, we define a probability distribution on $\on^X$ as follows. Let $\cl(X)$ be the closure of $X$ and let $\C(\cl(X))$ be all clauses $C$ such that $V(C) \subseteq \cl(X)$. Then, we define $$\nu_{\cl(X)}(x) = \frac{1}{Z} \cdot \Pi_{C \in \C(\cl(X))} \mu_C(x_{V(C)})$$ where $x_C$ denotes the coordinate of $x$ in $V(C)$. We can then set $\nu_X$ to be the marginal of $\nu_{\cl(X)}$ on to $X$.


The fact that $Z > 0$ (and thus the measures $\nu_{\cl(X)}$ above are well defined ) and that $\nu_X$ are locally consistent follows from the following lemma that was shown by \bnote{add lemma}

%The following theorem is follows from the proof of Theorem~3 in \cite{GMT09}.

\begin{lemma}
Let $P$ be a predicate of arity $k$ and $\mu$ be a pairwise independent distribuption over $P^{-1}(1)$.
Let $\eta, \delta > 0$.
Suppose a \MCSP$P$ instance $\I$ satisfies that for any collection $\mathcal C$
of constraints with $|\mathcal C| \leq \gamma n$, we have $|\partial(\mathcal
C)| \geq (k-2-\delta)$.
Then the family $\{ \nu_X \mid X \subseteq [n], |X| \leq T \}$ of local
distributions defined above is a $T$-round Sherali--Adams solution satisfying
all constraints on $\I$, where $T = ?$.
In particular, for any $R \subseteq S \subseteq [n], |S| \leq T$, the marginal
of $\nu_S$ on $R$ equals $\nu_R$.
Furthermore, for any closed subset $U = R\cup S$ with two components $R$ and
$S$, the marginal distribution of $\nu_U$ is the product distribution $\nu_R
\otimes \nu_S$.
\end{lemma}

%\begin{theorem}
%Let $P$ be a predicate of arity $k$ and $\mu$ be a pairwise independent distribuption over $P^{-1}(1)$.
%Let $\eta, \delta > 0$.
%Suppose a \MCSP$P$ instance $\I$ satisfies that for any collection $\mathcal C$
%of constraints with $|\mathcal C| \leq \gamma n$, we have $|\partial(\mathcal
%C)| \geq (k-2-\delta)$.
%Then there is a $T$-round Sherali--Adams solution satisfying all constraints on
%$\I$, where $T = \Omega(\delta\eta n/k)$.
%More precisely, there is a family $\{\mu_S\mid S \in {[n] \choose \leq T}\}$ of
%local distributions, such that $\mu_S$ is a distribution over assignments
%$\{\pm 1\}^S$ for every subset $S\subseteq [n]$ of size at most $T$.
%Further, this family satisfies the following properties:
%\begin{itemize}
%\item (Consistency) for any $S\in {[n] \choose \leq T}$ and any $R\subseteq S$,
%the marginal of $\mu_S$ on $R$ is exactly $\mu_R$.
%\item (Completeness) for any constraint $C$ in $\I$, $\mu_C$ equals $\mu$.
%\end{itemize}
%\end{theorem}

Since $\tE$ corresponds to a valid expectation locally, we obtain that $\tE$ induces a positive semidefinite (PSD) inner product on any space of functions of a small number of variables.
\begin{lemma}[Local PSDness]
Let $V \subseteq P_s^n$ be any subspace such that $V \subseteq \Span \{ \chi_A \mid A \subseteq T\}$ for some $T\subseteq [n]$, $|T| = o(n)$. Then, for every $f \in V$, $$\tE[ f^2] \geq 0.$$ \label{lem:local-PSD}
\end{lemma}

